Transfer Learning for LQR Control

In this paper, we study a transfer learning framework for Linear Quadratic Regulator (LQR) control, where (i) the dynamics of the system of interest (target system) are unknown and only a short trajectory of impulse responses from the target system is provided, and (ii) impulse responses are available from $N$ source systems with different dynamics. We show that the LQR controller can be learned from a sufficiently long trajectory of impulse responses. Further, a transferable mode set can be identified using the available data from source systems and the target system, enabling the reconstruction of the target system's impulse responses for controller design. By leveraging data from source systems, we show that the sample complexity for synthesizing the LQR controller can be reduced by $50 \%$. Algorithms and numerical examples are provided to demonstrate the implementation of the proposed transfer control framework.

==> preamble.tex <==
% This file defines the handy packages, notations, commands for .tex file
% To use this file, put this file in the same directory as the main .tex file, and add \input{preamble.tex} at the beginning
% Check LatexTemplate.tex for example illustrations

%%\usepackage[letterpaper, margin=1in]{geometry}
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{xcolor}
% \usepackage{appendix}
\usepackage{comment}
\usepackage{balance}


%-------------------------------------------- Packages for displaying Image------------------------------------------
\usepackage{graphicx}
\usepackage{subfig}
% \ifCLASSOPTIONcompsoc
% \usepackage[caption=false,font=footnotesize,labelfont=sf,textfont=sf]{subfig}
% \else
% \usepackage[caption=false,font=footnotesize]{subfig}
% \fi
\graphicspath{ {images/}}
% \usepackage{caption}
%--------------------------------------------------------------------------------------------------------------------

%----------------------------------------- Packages for Special Characters ------------------------------------------
\usepackage{pifont}
%--------------------------------------------------------------------------------------------------------------------

%%---------------------------------------------- Packages for Hyperlink ----------------------------------------------
 \usepackage{hyperref}
\hypersetup{
		colorlinks,
		 linkcolor={red!50!black},
		 citecolor={blue!50!black},
		 urlcolor={blue!80!black}
	}
% \usepackage[colorlinks,urlcolor=blue,linkcolor=blue,citecolor=blue]{hyperref} 
%
%\makeatletter
%\let\NAT@parse\undefined
%\makeatother
%\usepackage[colorlinks,urlcolor=blue,linkcolor=blue,citecolor=blue]{hyperref}
%%--------------------------------------------------------------------------------------------------------------------

%---------------------------------------------- Packages for Algorithm-----------------------------------------------
%\usepackage[ruled, vlined]{algorithm2e}
%\usepackage{algorithm2e}
\usepackage{algorithmic}

%--------------------------------------------------------------------------------------------------------------------

%------------------------------------------ Package for String Operation --------------------------------------------
% I use the \IfStrEq command to judge if the input is number ''1''.
\usepackage{xstring}
%--------------------------------------------------------------------------------------------------------------------

%%---------------------------------------------- Packages for Citations-----------------------------------------------
%\usepackage{cite}
%\usepackage[numbers]{natbib}
%\bibliographystyle{apalike} % Author+Year
%% If encounter issue "natbib Error: Bibliography not compatible with author-year citations", delete .aux and .bbl 
%% file and recompile.
%%--------------------------------------------------------------------------------------------------------------------

%%------------------------------------------ Packages for Bibliographic Entries --------------------------------------
%% Put what the text shows up in the reference list into the text
%\usepackage{bibentry}
%\nobibliography*
%%--------------------------------------------------------------------------------------------------------------------

%------------------------------------------------ Packages for Tables------------------------------------------------
\usepackage{multirow}
\usepackage{calc}
\usepackage{adjustbox}
\usepackage{booktabs}

% By default, in the table, the content in the cell tend to move up a little rather than stay in the middle, \mytabspace command can correct his
% This command will not change the row height, but only move the cell content.
% This command can only be applied to a specific cell
\newcommand{\mytabspace}[1]{%
	\parbox[c][\totalheightof{#1}+1\fboxsep+1\fboxrule][c]{\widthof{#1}}{#1}%
}

% Commands used to ENLARGE the top and bottom margin of an entire row, and the row height will increase accordingly
\newcommand\Tstrut{\rule{0pt}{3ex}}       
% "top" strut; Change the last variable to adjust the top margin of a row in the table
\newcommand\Bstrut{\rule[-1.5ex]{0pt}{0pt}} 
% "bottom" strut; Change the first variable to adjust the bottom margin of a row in the table, less frequently used.
\newcommand{\TBstrut}{\Tstrut\Bstrut} % top&bottom struts

\newcommand{\cellvcenter}[1]{\begin{tabular}{l} #1 \end{tabular}}
\usepackage{makecell}
%--------------------------------------------------------------------------------------------------------------------

%----------------------------- Packages for Theorems and Function -----------------------------------------

\usepackage{bbm}
\theoremstyle{plain}
\newtheorem{setup}{Setup}
\newtheorem{fact}{Fact}
\renewcommand*{\thesetup}{S\arabic{setup}}
\newtheorem{problem}{Problem}
\renewcommand*{\theproblem}{P\arabic{problem}}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
% \renewcommand*{\theassumption}{A\arabic{assumption}}

%\newtheorem*{definition*}{Definition}
%\newtheorem*{assumption*}{Assumption}
%\newtheorem*{problem*}{Problem}
%\newtheorem*{theorem*}{Theorem}
%\newtheorem*{lemma*}{Lemma}
%\newtheorem*{corollary*}{Corollary}
%\newtheorem*{proposition*}{Proposition}
%\newtheorem*{remark*}{Remark}
%
%% The following defines command that can customize theorem labelling
%\newtheorem{innercustomgeneric}{\customgenericname}
%\providecommand{\customgenericname}{}
%\newcommand{\newcustomtheorem}[2]{%
	%	\newenvironment{#1}[1]
	%	{%
		%		\renewcommand\customgenericname{#2}%
		%		\renewcommand\theinnercustomgeneric{##1}%
		%		\innercustomgeneric
		%	}
	%	{\endinnercustomgeneric}
	%}
%\newcustomtheorem{customtheorem}{Theorem}
%\newcustomtheorem{customlemma}{Lemma}
%\newcustomtheorem{customproposition}{Proposition}
%--------------------------------------------------------------------------------------------------------------------

%------------------------------ Package for Changing the Bullet Style of Enumerate ----------------------------------
\let\labelindent\relax
\usepackage{enumitem}
%\begin{enumerate}[label=(\roman*)]
%\item
%\end{enumerate}
%--------------------------------------------------------------------------------------------------------------------

%------------------------- Command for Allowing Align Environment to Break Between Pages ----------------------------
\allowdisplaybreaks
%\begin{align*}
%a\\
%b\\
%c\\
%d\\
%e\stepcounter{equation}\tag{\theequation}\label{eq_76}\\
%f\\
%g\\
%h\\
%i
%\end{align*}


%-------------------------------------------- Commands for Letters----------------------------------------
\input{preambleLettersDef.tex}
%--------------------------------------------------------------------------------------------------------------------



%------------------------------------------------- Common Math Operator ---------------------------------------------
\newcommand{\norm}[1]{\|{#1} \|}
\newcommand{\normauto}[1]{\left\|{#1} \right\|}
\newcommand{\normbig}[1]{\big\| #1 \big\|}
\newcommand{\normBig}[1]{\Big\| #1 \Big\|}
\newcommand{\normbigg}[1]{\bigg\| #1 \bigg\|}
\newcommand{\normBigg}[1]{\Bigg\| #1 \Bigg\|}
\newcommand{\crlbkt}[1]{\{ #1 \}}
\newcommand{\crlbktauto}[1]{\left\{ #1 \right\}}
\newcommand{\crlbktbig}[1]{\bigl\{ #1 \bigr\}}
\newcommand{\crlbktBig}[1]{\Bigl\{ #1 \Bigr\}}
\newcommand{\crlbktbigg}[1]{\biggl\{ #1 \biggr\}}
\newcommand{\crlbktBigg}[1]{\Biggl\{ #1 \Biggr\}}
\newcommand{\sqbkt}[1]{[ #1 ]}
\newcommand{\sqbktauto}[1]{\left[ #1 \right]}
\newcommand{\sqbktbig}[1]{\bigl[ #1 \bigr]}
\newcommand{\sqbktBig}[1]{\Bigl[ #1 \Bigr]}
\newcommand{\sqbktbigg}[1]{\biggl[ #1 \biggr]}
\newcommand{\sqbktBigg}[1]{\Biggl[ #1 \Biggr]}
\newcommand{\prnthauto}[1]{\left( #1 \right)}
\newcommand{\prnthbig}[1]{\bigl( #1 \bigr)}
\newcommand{\prnthBig}[1]{\Bigl( #1 \Bigr)}
\newcommand{\prnthbigg}[1]{\biggl( #1 \biggr)}
\newcommand{\prnthBigg}[1]{\Biggl( #1 \Biggr)}
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
% \newcommand{\indicator}{\mathbbm{1}}
\newcommand{\indicator}[1]{\mathbf{1}_{\crlbktauto{#1}}}

\newcommand{\st}{\textup{subject to}}
\newcommand{\mxz}{\textup{maximize}}
\newcommand{\mnz}{\textup{minimize}}

\newcommand{\wht}[1]{\widehat{#1}}		% Widehat
\newcommand{\wtd}[1]{\widetilde{#1}}	% Widetilde

\newcommand{\R}{\mathbb{R}}				% Real line R
\newcommand{\NaturalNum}{\mathbb{N}}				% Real line R
\newcommand{\dm}[2]
{
	\IfStrEq{#2}{1}{\R^{#1}}{\R^{#1 \x #2}}
}

\newcommand{\N}{\mathcal{N}}			% Normal Distribution N
\newcommand{\onevec}{\mathbf{1}} 		% Bold 1, All 1 vector

\newcommand{\rank}{\textup{{rank}}} 			% rank
\newcommand{\tr}{\textup{\textbf{tr}}} 			% Trace
\newcommand{\diag}{\textup{\textbf{diag}}} 		% Diag
\newcommand{\cond}{\textup{\textbf{cond}}} 		% Condition number
\newcommand{\vek}{\textup{\textbf{vec}}}			% Vectorization
\newcommand{\expctn}{\mathbb{E}} 	 	% Expectation
\newcommand{\cov}{\textup{\textbf{Cov}}}	 	% Expectation
\newcommand{\CRB}{Cram{\'e}r-Rao bound} % Expectation
\newcommand{\inv}{{-1}} 				% Superscript inverse
\newcommand{\invv}[1]{{\mskip-1mu \scalebox{1.5}[0.75]{-} \mskip-1mu #1}} %
\newcommand{\gotoinf}{\rightarrow \infty} 				% Superscript inverse
\newcommand{\prob}{\mathbb{P}} 				% The upright P to denote probability
\newcommand{\diff}{\textup{d}}				% The d in derivative
\newcommand{\fro}{\textup{F}}			% Subscript for Frobenius norm
\newcommand{\iiddist}{\overset{\textup{i.i.d.}}{\sim}}
\newcommand{\poly}{\textup{poly}}
\newcommand{\polylog}{\textup{polylog}}
\newcommand{\order}[1]{{\cal{O}}(#1)}

% Transpose
\usepackage{amssymb}
\makeatletter
\newcommand*{\T}{{\mathpalette\@transpose{}}}
\newcommand*{\@transpose}[2]{\raisebox{\depth}{$\m@th#1\intercal$}}
%\newcommand*{\@transpose}[2]{\raisebox{\depth}{$\m@th#1\top$}}
\makeatother

% The product x sign used in dimension, e.g. R^{m \x n}
% Compared with \times, \x can save more space before and after the operator
\newcommand*{\x}{\mathsf{x}\mskip1mu} 	

% The minus sign
% Compared with -, \m can save more space before and after the operator 
\newcommand*{\minus}{\mathsf{-}\mskip1mu} 

%--------------------------------------------------------------------------------------------------------------------

%---------------------------------------------------- Other Commands ------------------------------------------------
% Allow inline math equation to break at commas
\newcommand{\splitatcommas}[1]{%
	\begingroup
	\begingroup\lccode`~=`, \lowercase{\endgroup
		\edef~{\mathchar\the\mathcode`, \penalty0 \noexpand\hspace{0pt plus .1em}}%
	}\mathcode`,="8000 #1%
	\endgroup
}
% $\splitatcommas{
	%   \frac{1}{2},\frac{3}{5},\frac{8}{13},\frac{21}{34},\frac{55}{89},
	%   \frac{144}{233},\frac{377}{610},\frac{987}{1597},\frac{2584}{4181},
	%   \frac{6765}{10946},\frac{17711}{28657},\frac{46368}{75025},
	%   \frac{121393}{196418},\frac{317811}{514229},\frac{832040}{1346269},
	%   \frac{2178309}{3524578},\frac{5702887}{9227465},
	%   \frac{14930352}{24157817},\frac{39088169}{63245986},\frac{102334155}{165580141}
	% }$

% Allow the equation in itemize or enumerate to align with the item labe
\newcommand\Item[1][]{% 
\ifx\relax#1\relax  \item \else \item[#1] \fi
\abovedisplayskip=0pt\abovedisplayshortskip=0pt~\vspace*{-\baselineskip}}

% The following commands are for review responses
% initialize counters for reviewer number and comment number
\newcounter{reviewer}
\setcounter{reviewer}{0}
\newcounter{point}[reviewer]
\setcounter{point}{0}

\makeatletter
\newcommand{\customlabelfig}[2]{%
    \protected@write \@auxout {}{
    \string \newlabel {#1}{{#2}{\thepage}{#2}{#1}{}{}}
    }
}
\makeatother

\makeatletter
\newcommand{\customlabelresponse}[2]{%
   \protected@write \@auxout {}{
   \string \newlabel {#1}{{#2}{\thepage}{#2}{#1}{}} 
   }%
   \hypertarget{#1}{#2}
}
\makeatother



% Set the format of reviewer comment numbers and responses.
% \renewcommand{\thepoint}{Q\,\thereviewer.\arabic{point}} 
\renewcommand{\thepoint}{Q\,\arabic{point}} 
\newcommand{\point}[1]{\refstepcounter{point}  \bigskip \medskip \noindent {\fontseries{b}\selectfont \thepoint } \textit{#1}\par}
\newcommand{\reply}{\medskip \noindent \textbf{Reply}:\ }
\newcommand{\reviewerNumber}[1]{\refstepcounter{reviewer}  \bigskip \medskip \noindent \section*{#1} \par}

% Set the format for reviewer headings
\newcommand{\reviewersection}{\stepcounter{reviewer}
                  \section*{Response to Reviewer \thereviewer}}

